A Data-Efficient Approach to Behind-the-Meter Solar Generation Disaggregation

With the emergence of cost effective battery storage and the decline in the solar photovoltaic (PV) levelized cost of energy (LCOE), the number of behind-the-meter solar PV systems is expected to increase steadily. The ability to estimate solar generation from these latent systems is crucial for a range of applications, including distribution system planning and operation, demand response, and non-intrusive load monitoring (NILM). This paper investigates the problem of disaggregating solar generation from smart meter data when historical disaggregated data from the target home is unavailable, and deployment characteristics of the PV system are unknown. The proposed approach entails inferring the physical characteristics from smart meter data and disaggregating solar generation using an iterative algorithm. This algorithm takes advantage of solar generation data (aka proxy measurements) from a few sites that are located in the same area as the target home, and solar generation data synthesized using a physical PV model. We evaluate our methods with 4 different proxy settings on around 160 homes in the United States and Australia, and show that the solar disaggregation accuracy is improved by 32.31% and 15.66% over two state-of-the-art methods using only one real proxy along with three synthetic proxies. Furthermore, we demonstrate that using the disaggregated home load rather than the net load data could improve the overall accuracy of three popular NILM methods by at least 22%.

==> sections/DoNotEdit_methodology.tex <==
\section{methodology}
% \begin{figure}[t!]
%   \centering
%   \includegraphics[width=.75\linewidth]{imgs/neural_separation_v2.pdf}
%   \caption{Overview of the proposed solar disaggregation method.}
%   \label{fig:framework}
% \end{figure}

Our solar disaggregation method consists of two main steps: weight initialization and solar disaggregation.
In the weight initialization step, 
we use the net load data of the target customer and the solar generation data collected from proxies 
to initialize the weight vector $\textbf{w}$ of the solar mixture model.
Then in the disaggregation step, 
% inspired by the work of Kabir et al.~\cite{Kabir2019}, 
we iteratively estimate the home load and the solar generation until the parameters of our model converge.
We describe these two steps below.

\subsection{Weight Initialization}
A good initialization for the weights of the mixture model 
can enhance the performance of the disaggregation method and reduce its convergence time.
Our weight initialization method includes 3 main steps:
\begin{enumerate}
  \item Estimating the physical characteristics of PV systems of the target home and solar proxies.
  \item Finding the maximum solar generation of each PV system.
  \item Solving an optimization problem to determine the initial weight vector $\textbf{w}$.
\end{enumerate}
We use an open source toolkit, SolarTK~\cite{bashir2019},
to estimate the physical characteristics of PV systems including its tilt, orientation, and panel size.
To estimate these parameters, the toolkit takes as input real solar generation data 
and finds the maximum solar generation.
We can run this toolkit on proxy measurements, but we lack the real solar generation data from the target home.
To solve this problem, we approximate the solar generation of the target home given the net load data $\textbf{y}$ 
from this expression $\hat{\textbf{s}} \approx [l_{base} - \textbf{y}]^+$, 
where $[~~]^+$ is an operator that truncates negative elements of a vector to zero, 
and $l_{base}$ is the target home's base power consumption calculated as the minimum consumption level at night time.
SolarTK is then applied to the estimated solar generation of the target home and 
the real solar generation of solar proxy/proxies 
to obtain the estimated parameters for all PV systems.
Since we use a city's longitude and latitude as a approximate location for all the PV systems located in it, 
the estimated parameters may not be highly accurate.

We then calculate the maximum solar generation for each proxy and target home 
using the estimated deployment characteristics obtained in Step~1.
The maximum solar generation is the potential generation of a PV system under clear sky condition, 
that is determined by the system's physical characteristics, the ambient temperature and the location of PV.
We denote the maximum solar generation of the $k^{\text{th}}$ proxy by $\textbf{m}^{p}_{k}\in\mathbb{R}^{T}$,
and the maximum solar generation of target home by $\textbf{m}^{c}\in\mathbb{R}^{T}$.

In the last step, we utilize the idea of solar transposition model 
to determine the initial weight vector $\textbf{w}$ for the solar mixture model.
In~\cite{Shaker2016}, the authors transpose the metered solar generation to estimate the solar generation of unknown target PV site by utilizing the system-specific information (e.g. exact location and PV capacity). Formally, 
\begin{align} 
\textbf{s}_{target} = \alpha \cdotp \textbf{s}_{proxy}
\label{fun:transposition_in_our_format}
\end{align}
where $\alpha$ is a function that depends on time, location and other site-specific factors.
In our method, we simplify $\alpha$ as a constant weight factor.
Since we do not have the true solar generation from target home in Equation~(\ref{fun:transposition_in_our_format}),
we use the maximum solar generations to determine the initial weight of each solar proxy.
Then, the weight factor $\textbf{w}_k$ for the $k^{\text{th}}$ proxy can be determined by solving the following optimization problem: 
\begin{equation}
\begin{aligned}
% &\min_{w_{k}} &\sum_{t=0}^{T}(MaxS_i(t) - \textbf{w}_{i,k} \times MaxP_k(t))^2 \\
&\min_{\textbf{w}_k} & \| \textbf{w}_k\cdotp\textbf{m}^p_k - \textbf{m}^{c}\|_2 \\
&\textrm{subject to} & \textbf{w}_k > 0  %\succeq 0
\label{fun:determine_weight}
\end{aligned}
\end{equation}

\subsection{Solar Disaggregation}
\label{subsection:solar_disaggregation}
We now present our solar disaggregation method and describe the features and models for home load and solar estimation.
\begin{figure*}[ht]
  \includegraphics[width=\textwidth, height=3cm]{imgs/real_solar_gen_pecan_summer.png}
  \caption{The solar generation of 19 homes in the Pecan Street dataset over 2 weeks. 
  The thicker line shows the average solar generation across all the homes.}
  \label{fig:real_solar}
\end{figure*}

\textbf{Solar mixture model:} As previously mentioned, we use the generation of solar proxies as the solar-related features and apply a linear model to estimate the solar generation of the target home.
The motivation behind using a linear model is that, 
as Figure~\ref{fig:real_solar} shows, 
the solar generations from city-wide or neighborhood-wide PV systems show a similar pattern.
However, there are two challenges we have to address if we use a linear model for estimating the solar generation of the target homes.
First, there are still nonlinear differences between the solar proxies and solar generation of the target homes.
To reduce these errors, we use multiple proxies with different parameters from different locations.
Second, the generation data from a large number of solar proxies might not be available in practice.
To address this problem, we combine the real solar proxies with synthetic solar proxies created using a physical PV system model and environmental measurements.
The physical PV model we used for synthetic proxy is based on the PV performance modeling collaborative~\cite{PVPMC} and PVWatts~\cite{PVWatts}.
The output power of the PV model with the specified rating $P_{dc0}$ in equation (\ref{fun:PVWatts_model}) can be computed given the transmitted plane of array (POA) irradiance $I_{tr}$ and cell temperature $T_{cell}$. 
% Then we can calculate AC output power given DC output power.
\begin{align}
P_{dc} = \frac{I_{tr}}{E_{ref}}P_{dc0}(1+\gamma(T_{cell} - T_{ref}))
\label{fun:PVWatts_model}
\end{align}
where $\gamma$, $E_{ref}$ and $T_{ref}$ are known parameters.
$I_{tr}$ is determined by solar irradiance data (direct normal irradiance, diffuse horizontal irradiance, global horizontal irradiance), PV system characteristics (e.g. tilt, orientation) and location information.
$T_{cell}$ requires wind speed, ambient air temperature and solar irradiance data. 
We use different preset technical parameters for different synthetic proxies.

\textbf{Home load model:} To estimate the home load, we use a random forest regression model 
which is a supervised learning algorithm that uses ensemble learning method for regression.
We use scikit-learn~\cite{scikit} python library to implement the load model.
This regression model is widely used to utilize the effects of explanatory variables, such as temperature and time of day, to estimate the home load.
We use 4 non-customer-specific explanatory variables as our load related features $\textbf{X}^L$ for all customers. 
These variables include the temperature $\textbf{c}$, the weighted moving average of temperature over the last 24 hours $\textbf{c}_{wmv}$, hour of the day $\textbf{h}$ and a binary variable $\textbf{d}$ to indicate week day or weekend. 
Thus, we have $\textbf{X}^{L} = [\textbf{c}, \textbf{c}_{wmv}, \textbf{h}, \textbf{d}]$.

\input{sections/algorithm}
\textbf{Disaggregation algorithm:} 
Algorithm~\ref{alg:solar_dis} is the pseudocode of the proposed solar disaggregation algorithm.
After obtaining the initial weights $\textbf{w}$ for the solar mixture model, 
we first estimate the solar PV generation $\textbf{s}^{iter}$ using a linear combination of the solar proxies.
% For any fixed solar generation $S_{i}^{iter}$, 
Then, we use $\textbf{y} = \hat{\textbf{l}} - \hat{\textbf{s}}$ to calculate the estimated home load $\textbf{l}^{iter}$ (line 2) and incrementally train the load model using $\textbf{l}^{iter}$ and load related features $\textbf{X}^L$ (line 3).
Based on the updated home load $\textbf{l}^{iter}$ (line 4), we determine solar generation $\textbf{s}^{iter}$ (line 5), 
update the weights for solar proxies (line 6), and recalculate the solar generation using the updated weights (line 7). 
We repeat the above steps until the solar proxy weights $\textbf{w}$ converge or we reach the maximum number of iterations.
